Efficient And Portable SDR Waveform Development: The Nucleus Concept

Future wireless communication systems should be flexible to support different waveforms (WFs) and be cognitive to sense the environment and tune themselves. This has lead to tremendous interest in software defined radios (SDRs). Constraints like throughput, latency and low energy demand high implementation efficiency. The tradeoff of going for a highly efficient implementation is the increase of porting effort to a new hardware (HW) platform. In this paper, we propose a novel concept for WF development, the Nucleus concept, that exploits the common structure in various wireless signal processing algorithms and provides a way for efficient and portable implementation. Tool assisted WF mapping and exploration is done efficiently by propagating the implementation and interface properties of Nuclei. The Nucleus concept aims at providing software flexibility with high level programmability, but at the same time limiting HW flexibility to maximize area and energy efficiency.

==> mapping.tex <==
\section{Mapping and Evaluation}
\label{sec:mapping}

The waveform description (in terms of nuclei and non-nuclei tasks) and the nuclei-implementation from the BSP form the basis of waveform mapping onto the HW platform. Even though the implementations of the nuclei are efficient, the overall system performance is not guaranteed and it is heavily influenced by the spatial and temporal mapping.

Figure ~\ref{fig:wde} sketches the scenario of spatial mapping for a given HW platform. The first subscript of nucleus implementation (NI) denotes the nuclei-API and second subscript denotes the PE for which the implementation is available in the BSP. Therefore, NI25 denotes the NI of nucleus 2 on PE 5. The key difference to the traditional waveform spatial mapping is that the task from the waveform description is mapped not to the HW PE, but to the available nucleus implementation from the BSP. As shown in Figure 3.1, there might be several choices for selection depending on the BSP.
\begin{itemize}
\item For one nucleus, there can be several NIs on one PE.
\item For one nucleus, there can be several NIs on several PEs.
\item On one PE, there can be NIs for different nuclei.
\item The implementations can come from different vendors.
\end{itemize}

The choice of the NI will be based not only on the performance but also on the data structure of the neighboring NI interfaces. The non-nuclei (NNI) tasks, which represent computationally light tasks, might be mapped to the general purpose core (PE4) as shown in Figure 3.1.

One or more nuclei (and/or non-nuclei) tasks can be mapped onto a single PE. This requires temporal mapping/scheduling of the tasks depending on the data dependencies. We believe that scheduling will be static, at least for the critical physical layer processing kernels which are our focus. The scheduling information can be derived from the waveform description and the tasks can be scheduled accordingly. Further evaluation is needed to make sure that the constraints of the waveform are met.
The mapping challenge is to identify the right choice of NIs that are not only compatible to each other and meet the requirements of the waveform but also maximize the overall system efficiency. Therefore, the properties of the nuclei and NIs have to be captured in a way that enables future tool based mapping and exploration of the waveform.

Detailed evaluation of the mapping decisions is necessary not only to check if the waveform constraints are met but also to maximize system performance. The waveform constraints can be verified in terms of latency, throughout, BER and critical loops. To maximize total system performance, metrics are needed with which different decisions can be evaluated. The following metrics can be used for mapping:
\begin{itemize}
\item Increasing data localization
\item Minimizing communication
\item Minimizing synchronization
\item Maximizing PE utilization
\end{itemize}
It is clear that the mapping exploration should be done in an iterative manner and at different abstraction levels to gain more accuracy. The WDE should provide the infrastructure necessary for doing the exploration and simulation for evaluating the mapping decisions.

